MQT-TZ: Hardening IoT Brokers Using ARM TrustZone

The publish-subscribe paradigm is an efficient communication scheme with strong decoupling between the nodes, that is especially fit for large-scale deployments. It adapts natively to very dynamic settings and it is used in a diversity of real-world scenarios, including finance, smart cities, medical environments, or IoT sensors. Several of the mentioned application scenarios require increasingly stringent security guarantees due to the sensitive nature of the exchanged messages as well as the privacy demands of the clients/stakeholders/receivers. MQTT is a lightweight topic-based publish-subscribe protocol popular in edge and IoT settings, a de-facto standard widely adopted nowadays by the industry and researchers. However, MQTT brokers must process data in clear, hence exposing a large attack surface. This paper presents MQT-TZ, a secure MQTT broker leveraging Arm TrustZone, a trusted execution environment (TEE) commonly found even on inexpensive devices largely available on the market (such as Raspberry Pi units). We define a mutual TLS-based handshake and a two-layer encryption for end-to-end security using the TEE as a trusted proxy. The experimental evaluation of our fully implemented prototype with micro-, macro-benchmarks, as well as with real-world industrial workloads from a MedTech use-case, highlights several trade-offs using TrustZone TEE. We report several lessons learned while building and evaluating our system. We release MQT-TZ as open-source.

==> figs/handshake-algorithm.tex <==
\begin{algorithm}[t!]
    \floatname{Protocol}{Two-Step Handshake}
    \renewcommand{\thealgorithm}{}
    \caption{Steps that Mallory follows to hjobtain key K}
    \label{protocol1}
    \begin{algorithmic}[1]
    \STATE $M$ : Eavesdrops the protocol 1 above and gets $X$ from step 1 and initiates the same protocol with $B$, by substituting $X$ for $K$ above.
    \STATE $M\rightarrow{B}$ : $P = E_{B}(S_{M}(X)) = E_{B}(S_{M}(E_{B}(S_{A}(K))))$
    \STATE $B$ : $V_{M}(D_{B}(P)) = V_{A}(D_{B}(E_{B}(S_{A}(X)))) = X$
    \STATE $B\rightarrow{M}$ : $Q = E_{M}(S_{B}(X)) = E_{M}(S_{B}(E_{B}(S_{A}(K))))$\\
    Since the same key pair is used for both encryption and signing, $S_{B}(E_{B}(message)) = message$\\
    Therefore, $Q = E_{M}(S_{A}(K))$
    \STATE $M$ : $D_{M}(Q) = S_{A}(K)$
    \STATE $M$ : Since the same key pair is used for both encryption and signing, $E_{A}(S_{A}(K)) = K$. Mallory can obtain the key $K$ in this way and decrypt all the subsequent messages encrypted with key $K$.
    \end{algorithmic}
\end{algorithm} 


==> figs/mqt-tz-architecture.tex <==
\begin{tikzpicture}
    \definecolor{blue0}{RGB}{0,25,51}
    \definecolor{blue1}{RGB}{0,51,102}
    \definecolor{blue2}{RGB}{0,128,255}
    \definecolor{blue3}{RGB}{153,204,255}
    \definecolor{yellow}{RGB}{250,165,25}
    \definecolor{lightyellow}{RGB}{229,208,66}

    % MQTT Broker
    % Non-Secure
    \draw[preaction={fill,white},pattern=dots,pattern color=gray!40] (2.5, 1) rectangle (9.5, 5);
    \draw[preaction={fill,white},pattern=crosshatch,pattern color=gray!40] (2.5, 5) rectangle (9.5, 8.25);
    
    % Lines for decrypt
    % \draw[->, very thick, red!50!black] (1, 6.1) -- (0.35, 6.1) -- (0.35, 4.25);
    % \draw[->, very thick, green!50!black] (0.35, 3.75) -- (0.35, 3) -- (3, 3);
    % \draw[->, very thick, red!50!black] (6, 4.25) -- (6, 6.1) -- (5.65, 6.1);
    % \draw[->, very thick, green!50!black] (6, 3.25) -- (6, 3.75);
    % Lines for encrypt
    % \draw[->, very thick, red!50!black] (6.5, 4.25) -- (6.5, 6.1) -- (6.95, 6.1);
    % \draw[->, very thick, green!50!black] (6.5, 3.25) -- (6.5, 3.75);
    % \draw[->, very thick, red!50!black] (11.5, 6.1) -- (12.15, 6.1) -- (12.15, 4.25);
    % \draw[->, very thick, green!50!black] (12.15, 3.75) -- (12.15, 3) -- (9, 3);
    % MQTT Broker Module
    \draw[fill=white] (3, 3.75) rectangle (9, 8.00) node[pos=.5,yshift=47pt] {\texttt{\textbf{\Large MQT-TZ Message Broker}}};
    \draw[fill=gray!10, align=center] (3.5, 5.75) rectangle (4.0, 7) node[pos=.5] {\texttt{A} \\ \texttt{C} \\ \texttt{L}};
    \draw[fill=gray!10, align=center] (4.5, 5.75) rectangle (5.75, 7) node[pos=.5] {\texttt{MQTT} \\ \texttt{DB}};
    \draw[fill=gray!10, align=center] (6.5, 5.75) rectangle (8.5, 7) node[pos=.5] {\texttt{\textbf{\small Re-encryption}} \\ \texttt{\small \textbf{TA} (REE)}};
    \draw[fill=gray!10, align=center] (3.5, 4.00) rectangle (8.5, 4.5) node[pos=.5] {\texttt{\textbf{Re-encryption TA} (TEE)}};
    \draw[->, dotted, thick] (7, 5.75) -- (7, 4.5) node[pos=.8, anchor=east] {\includegraphics[width=0.2cm]{images/lock.png}} node[pos=.8, anchor=west] {\blackcircled{4}};
    \draw[<-, dotted, thick] (7.75, 5.75) -- (7.75, 4.5) node[pos=.8, anchor=west] {\includegraphics[width=0.2cm]{images/lock.png} \blackcircled{8}};
    \draw[->, thick] (4.5, 4) -- (4.5, 3.25) node[pos=.57, anchor=west] {\blackcircled{5}};
    \draw[<-, thick] (7.5, 4) -- (7.5, 3.25) node[pos=.57, anchor=east] {\blackcircled{7}};
    % SMC
    \draw[fill=white] (2.5, 5) rectangle (9.5, 5.5) node[pos=.5] {\textbf{\texttt{Secure Monitor Mode}}};
    % Secure Cache
    \draw[fill=gray!10] (3, 2.75) rectangle (9, 3.25) node[pos=.5] {\texttt{\textbf{Lightweight Secure World Cache}}};
    \draw[fill=white] (3, 2.25) rectangle (9, 2.75) node[pos=.5] {\texttt{Trusted Application Heap Memory}};
    \node at (6, 2) {\small{\texttt{Cache Page Miss (LRU)}}};
    \draw[->, thick] (3.5, 2.25) -- (3.5, 1.75) node[pos=.5, anchor=west] {\blackcircled{6}};
    \draw[<-, thick] (4, 2.25) -- (4, 1.75);
    \draw[->, thick] (8.5, 2.25) -- (8.5, 1.75) node[pos=.5, anchor=east] {\blackcircled{6}};
    \draw[<-, thick] (8, 2.25) -- (8, 1.75);
    % REE FS
    \draw[fill=gray!30] (3, 1.25) rectangle (9, 1.75) node[pos=.5] {\texttt{Tamper Proof Secure Storage}};
    % \draw[fill=white] (3, 0.25) rectangle (9, 1.25);
    % Grid
%    \draw[fill=gray!5] (3, 0.25) rectangle (3.9, 0.75);
%    \draw[fill=gray!5] (3.9, 0.75) rectangle (5, 1.25);
%    \draw[fill=gray!5] (5, 0.25) rectangle (5.95, 0.75);
%    \draw[fill=gray!5] (5.95, 0.75) rectangle (7.05, 1.25);
%    \draw[fill=gray!5] (7.05, 0.25) rectangle (8, 0.75);
%    \draw[fill=gray!5] (8, 0.75) rectangle (9, 1.25);
%    % Labels
%    \node[align=left] at (5.35, 0.75) {\small{\texttt{cl\_1} \hspace{2pt} \texttt{SK\textsubscript{cl\_1}}} \hspace{5pt} \small{\texttt{cl\_3} \hspace{2pt} \texttt{SK\textsubscript{cl\_3}} \hspace{5pt} $\dots$} \\
%    \small{\texttt{cl\_2} \hspace{2pt} \texttt{SK\textsubscript{cl\_2}}} \hspace{5pt} \small{\texttt{cl\_4} \hspace{3pt} \texttt{SK\textsubscript{cl\_2}}}};

    % MQTT Publisher
    \node at (1, 6.4) (mqtt-pub) {\includegraphics[width=1.2cm]{images/mosquitto_client_bw.png}};
    %\node at (mqtt-pub.south) {\small{\texttt{(cl\_1, t1)}}};
    % TLS Lines
    \draw[->, very thick, dashed] (mqtt-pub.east) -- (3.5, 6.4) node[pos=.5, anchor=south] {\includegraphics[width=0.2cm]{images/lock.png}} node[pos=.57, anchor=north] {\blackcircled{1}};
    %\node[anchor=north] at (2, 6.4) {\blackcircled{1}};
    \draw[->, dotted, thick] (4, 6.4) -- (4.5, 6.4) node[pos=.5, anchor=south] {\includegraphics[width=0.2cm]{images/lock.png}} node[pos=.5, anchor=north] {\blackcircled{2}};
    \draw[->, dotted, thick] (5.75, 6.8) -- (6.5, 6.8) node[pos=.5, anchor=south] {\includegraphics[width=0.2cm]{images/lock.png}} node[pos=.5, anchor=north] {\blackcircled{3}};
    \draw[->, dotted, thick] (5.75, 5.9) -- (6.5, 5.9) node[pos=.5, anchor=south] {\includegraphics[width=0.2cm]{images/lock.png}};
    %\node at (-2, 7) {}};

    % MQTT Subscribers
    \node at (11.0, 6.8) (mqtt-sub-top) {\includegraphics[width=1.2cm]{images/mosquitto_client_bw.png}};
    \draw[->, very thick, dashed] (8.5, 6.8) -- (mqtt-sub-top.west) node[pos=.5, anchor=south] {\includegraphics[width=0.2cm]{images/lock.png}};
    \node at (8.7, 6.35) {\blackcircled{9}};
    \node at (11.0, 3.5) (mqtt-sub-bottom) {\includegraphics[width=1.25cm]{images/hdd.png}};
    \draw[very thick, dashed] (8.5, 5.9) -- (9.8, 5.9);% node[pos=.5, anchor=south] {\includegraphics[width=0.2cm]{images/lock.png}};
    \draw[very thick, dashed] (9.8, 5.9) -- (9.8, 3.5) node[pos=.5, anchor=west] {\includegraphics[width=0.2cm]{images/lock.png}};
    \draw[->, very thick, dashed] (9.8, 3.5) -- (mqtt-sub-bottom.west);
    %\node at (mqtt-sub-bottom.south) {\small{\texttt{(cl\_3, SK\textsubscript{cl\_3})}}};
    % TLS Sub
    %\node[anchor=south] at (13.25, 7) {\texttt{TLS}};
    %\node[anchor=north] at (13.25, 7) {\includegraphics[width=0.3cm]{images/lock.png}};
    %\draw[->, very thick, dashed] (11.5, 7) -- (13.25, 7) -- (13.25, 6) -- (13.75, 6);
    %\draw[->, very thick, dashed] (11.5, 7) -- (13.25, 7) -- (13.25, 2) -- (13.75, 2);

    % CA
    %\draw[fill=gray!40] (0, 9) rectangle (12, 9.5) node[pos=.5] {\texttt{Let's Encrypt} - Certificate Authority};
    %\draw[dashed, ->] (-5, 9) -- ($(mqtt-pub.north) - (0, 14pt)$) node[pos=.5, anchor=west] {\texttt{Cert\textsubscript{Broker}}};
    %\draw[dashed, ->] (15, 9) -- ($(mqtt-sub-top.north) - (0, 14pt)$) node[pos=.5, anchor=west] {\texttt{Cert\textsubscript{Broker}}};
    %\draw[dashed, ->] ($(mqtt-sub-top.south) - (0, 12pt)$) -- ($(mqtt-sub-bottom.north) - (0, 14pt)$) node[pos=.5, anchor=west] {\texttt{Cert\textsubscript{Broker}}};

    % Legend
    %\draw[fill=gray!40] (0, 9) rectangle (12, 9.5) node[pos=.5] {\texttt{Let's Encrypt} - Certificate Authority};
    \draw[preaction={fill,white},pattern=dots,pattern color=gray!40] (1, 0.25) rectangle (1.5, 0.5) node[anchor=west,yshift=-4pt,align=center] {\footnotesize \texttt{Trusted Execution} \\[-5pt] \footnotesize \texttt{Environment}};
    \draw[preaction={fill,white},pattern=crosshatch,pattern color=gray!40] (1, -0.25) rectangle (1.5, 0) node[anchor=west,yshift=-4pt,align=center] {\footnotesize \texttt{Rich Execution} \\[-5pt] \footnotesize \texttt{Environment}};
    \draw[->, very thick, dashed] (4, 0.375) -- (4.5, 0.375) node[pos=.5, anchor=south] {\includegraphics[width=0.15cm]{images/lock.png}};
    \node[anchor=west] at (4.6, 0.375) (je) {\small \texttt{TLS \& App. Layer Encryption}};
    \draw[->, dotted, thick] (4, -0.125) -- (4.5, -0.125) node[pos=.5, anchor=south] {\includegraphics[width=0.15cm]{images/lock.png}};
    \node[anchor=west] at (4.6, -0.125) (je) {\small \texttt{Application Layer Encryption}};
    \draw[->, thick] (8.7, 0.375) -- (9.2, 0.375) node[anchor=west] {\small \texttt{Data in Clear}};


\end{tikzpicture}


==> figs/tls-handshake.tex <==
\begin{sequencediagram}
    \newthread{cli}{Client}
    \newinst[1]{ca}{CA (Let's Encrypt)}
    \tikzstyle{inststyle}+=[top color=gray!30, bottom color=gray!30]
    \newinst[1]{b-ns}{Broker (NS)}
    \tikzstyle{inststyle}+=[top color=gray!60, bottom color=gray!60]
    \newinst{b-s}{Broker (S)}
    \begin{sdblock}{TLS-HS}{TLS Handshake - Broker (Server) Authentication Only}
        \begin{call}{cli}{\small{\texttt{Hello(cliTLSProps)}}}{b-ns}{\small{\texttt{Hello(chosenTLSProps, brkCert)}}}
        \end{call}
        \begin{call}{cli}{\small{\texttt{Trust(brkCert)}}}{ca}{\small{\texttt{Y/N}}}
        \end{call}
    \end{sdblock}
    %\begin{sdblock}{\tiny{\texttt{Key Exchange}}}{\tiny{\texttt{Key Exchange}}}
    \begin{sdblock}{Cli-Auth}{Client Authentication w/ TZ-Specific Key over MQTT}
        \begin{call}{cli}{\small{\texttt{Enc(cliSK,brkPK)}}}{b-ns}{\small{\texttt{FW(data)}}}
            \begin{call}{b-ns}{\small{\texttt{FW(data)}}}{b-s}{\hspace{15pt} \parbox[t]{2cm}{\small \texttt{Enc(OK,} \\ \small \texttt{ cliSKey)}}}
                %\begin{call}{b-s}{\tiny{\texttt{Dec(encData,brkpK)}}}{b-s}{}
                \begin{call}{b-s}{\parbox[t]{3cm}{\small \texttt{Dec(encData,}\\ \small \texttt{ brkPK)}}}{b-s}{}
                \end{call}
                \begin{call}{b-s}{\small{\texttt{Store(cliSK)}}}{b-s}{}
                \end{call}
            \end{call}
        \end{call}
    \end{sdblock}
\end{sequencediagram}

